TransAug: Translate as Augmentation for Sentence Embeddings

While contrastive learning greatly advances the representation of sentence embeddings, it is still limited by the size of the existing sentence datasets. In this paper, we present TransAug (Translate as Augmentation), which provide the first exploration of utilizing translated sentence pairs as data augmentation for text, and introduce a two-stage paradigm to advances the state-of-the-art sentence embeddings. Instead of adopting an encoder trained in other languages setting, we first distill a Chinese encoder from a SimCSE encoder (pretrained in English), so that their embeddings are close in semantic space, which can be regraded as implicit data augmentation. Then, we only update the English encoder via cross-lingual contrastive learning and frozen the distilled Chinese encoder. Our approach achieves a new state-of-art on standard semantic textual similarity (STS), outperforming both SimCSE and Sentence-T5, and the best performance in corresponding tracks on transfer tasks evaluated by SentEval.

==> tables/transfer.tex <==
%!TEX root = ../emnlp2021.tex

\begin{table*}[ht]
    \begin{center}
    \centering
    \small
    %\resizebox{0.7\textwidth}{!}{%

    \begin{tabular}{lcccccccc}
    \toprule
       \tf{Model} & \tf{MR} & \tf{CR} & \tf{SUBJ} & \tf{MPQA} & \tf{SST} & \tf{TREC} & \tf{MRPC} & \tf{Avg.}\\
    \midrule
    \midrule
        \multicolumn{9}{c}{\it{Supervised models}}\\
    \midrule
        InferSent-GloVe$^\clubsuit$ & 81.57 & 86.54 & 92.50 & {90.38} & 84.18 & 88.20 & 75.77 & 85.59\\
        Universal Sentence Encoder$^\clubsuit$ & 80.09 & 85.19 & 93.98 & 86.70 & 86.38 & {93.20} & 70.14 & 85.10  \\
        \midrule
        SBERT\ba$^\clubsuit$ & \tf{83.64}&	\tf{89.43}&	94.39&	\tf{89.86} &	\tf{88.96}&	\tf{89.60}&	76.00&	\tf{87.41}\\ % original
        $*$ \ours-BERT\ba  & 82.69&	89.25&	\tf{94.81}&	89.59&	87.31&	88.40&	73.51&	86.51\\
        \tableindent w/ MLM & 82.68&	88.88&	94.52&	89.82&	88.41&	87.60&	\tf{76.12}&	86.86 \\
        \midrule
        SRoBERTa\ba & 84.91&	90.83&	92.56&	88.75&	90.50&	88.60&	\tf{78.14}&	87.76\\ % original model
        $*$ \ours-RoBERTa\ba  & 84.92&	\tf{92.00}&	\tf{94.11}&	\tf{89.82}&	91.27&	88.80&	75.65&	88.08\\ 
        \tableindent w/ MLM & \tf{85.08}&	91.76&	94.02&	89.72&	\tf{92.31}&	\tf{91.20}&	76.52&	\tf{88.66}\\
        $*$ \ours-RoBERTa$_{\texttt{large}}$ & 88.12&	92.37&	95.11&	90.49&	92.75&	91.80&	76.64&	89.61\\
        \tableindent w/ MLM & \tf{88.45}&	\tf{92.53}&	\tf{95.19}&	\tf{90.58}&	\tf{93.30}&	\tf{93.80}&	\tf{77.74}&	\tf{90.23} \\
    \bottomrule
    \end{tabular}
    % }
    \end{center}

    \caption{
        Transfer task results of different sentence embedding models (measured as accuracy). $\clubsuit$: results from \citet{reimers-gurevych-2019-sentence};
        $\heartsuit$: results from \citet{zhang-etal-2020-unsupervised}. We highlight the highest numbers among models with the same pre-trained encoder. MLM: adding MLM as an auxiliary task with $\lambda = 0.1$. 
    }
    \label{tab:main_transfer}
\end{table*}

